Harnessing the Web and Knowledge Graphs for Automated Impact Investing Scoring

The Sustainable Development Goals (SDGs) were introduced by the United Nations in order to encourage policies and activities that help guarantee human prosperity and sustainability. SDG frameworks produced in the finance industry are designed to provide scores that indicate how well a company aligns with each of the 17 SDGs. This scoring enables a consistent assessment of investments that have the potential of building an inclusive and sustainable economy. As a result of the high quality and reliability required by such frameworks, the process of creating and maintaining them is time-consuming and requires extensive domain expertise. In this work, we describe a data-driven system that seeks to automate the process of creating an SDG framework. First, we propose a novel method for collecting and filtering a dataset of texts from different web sources and a knowledge graph relevant to a set of companies. We then implement and deploy classifiers trained with this data for predicting scores of alignment with SDGs for a given company. Our results indicate that our best performing model can accurately predict SDG scores with a micro average F1 score of 0.89, demonstrating the effectiveness of the proposed solution. We further describe how the integration of the models for its use by humans can be facilitated by providing explanations in the form of data relevant to a predicted score. We find that our proposed solution enables access to a large amount of information that analysts would normally not be able to process, resulting in an accurate prediction of SDG scores at a fraction of the cost.

==> scratch.tex <==

\paragraph{Sustainability reports and Wikipedia descriptions} Majority of the organizations' sustainability reports only contain a few sentences concerning each SDG, and the relevant features (key words/phrases) for forecasting SDG scores make up an extremely low percentage of total features in text representation models like BoW. To discover SDG-relevant sentences in a company's sustainability report, we create a semantic search engine utilizing a query comprised of the concatenated keywords\footnote{The keywords list is available at this link: \url{https://drive.google.com/file/d/1IJIUvS9tydCMxHE0T45OePGNCx7v9Q6r/view?usp=sharing}} acquired from the Sustainable Development Solutions Network\footnote{\url{https://www.unsdsn.org/about-us}}. However, relevant is not enough to indicate that a company is contributing to a specific SDG objective, since many corporations try to green-wash their reports by incorporating SDG definitions. To find sentences that include evidence of a company's contribution to SDG goals, we use Natural Language Inference (NLI) to assess if the relevant sentences show the firm is helping achieve each SDG's goal. A sample of summarized key actions among companies for SDG 13 is shown in Table \ref{tab:Sample of summarized key actions for SDG 13: Climate Actions}. The number of companies with evidence found for each of the 17 SDGs could be found in Figure \ref{fig:Number of companies with evidence found for 17 SDGs}. Similarly, the company's business descriptions are retrieved by a search engine in response to a query for its products, services, and materials. A sample of business descriptions extracted from Wikipedia for companies is shown in Table \ref{tab:Wikipedia product information (sample)}.\\

\paragraph{News} 
The news is a reliable indicator of a company's operational operations. Because corporations like Amazon may surface frequently in social media, we decide to select the most significant company news. To measure the significance of the news, we create an aggregated sentiment score that takes into account sentiment, amplitude of sentiment, and the number of times the company is referenced in the news. 
\begin{align*}
    &\underline{aggregated sentiment score} = \underline{sentiment} \times \underline{magnitude of sentiment} \\&\times \underline{number of times the company is mentioned in the news article}
\end{align*}
The top 5 news with the highest and lowest aggregated sentiment scores are selected as the most influential for a company. In addition, a threshold of 0.55 matched words in the headline is set to filter out the news describing the same event.



\paragraph{Wikidata subgraph}
After obtaining the Wikidata subgraph with relation types of our interests,  we assemble a new corporate graph with only our interest companies. First, we compute the minimal distance between companies. 0.02 percent of company pairs are reachable in one step (directly connected), while 84.04 percent are reachable in two. If two companies are within 2 steps, we connect them. We know that the linkages between companies weaken when the threshold is raised. We chose 2 as the threshold since there are other companies in the knowledge graph that are not in our interests but could be direct suppliers or shareholders of companies in our interests. This new network is less dense than the Wikidata subgraph we obtained, as shown in Figure \ref{fig:degree_dist} and Figure \ref{fig:degree_dist2} that the node distribution is less spiky and more spread out compared to the Wikidata subgraph.


\subsubsection{Imbalanced classification of SDG scores}
% We want to determine how effectively our dataset can predict the given RobecoSAM SDG scores before we can extend the model to forecast a wider selection of stocks. As can be seen from Figure \textbf{TODO} for the distribution of the RobecoSAM SDG scores, we have an imbalanced classification problem due to the majority of firms have a neutral score while the other classes have very limited amount of samples. The three major models involved in classifying SDG scores are Balanced Random Forest (BRF),
% Graph Convolution Networks (GCN). BRF is used to firstly explore what types of textual information from our dataset is most useful in predicting SDG scores. Robeco provides the data for sector classification\footnote{GICS is developed by MSCI and Standard \& Poor's to classify companies to different sectors and industries: \url{https://en.wikipedia.org/wiki/Global_Industry_Classification_Standard}} in 69 industries of a company which is used as the benchmark feature. Graph classification algorithms GCN is used to explore whether the information contained in the corporate graph we constructed from Wikidata subgraph could contribute to forecasting SDG scores besides the textual features. 
Before expanding the model to anticipate other companies, we want to see how well our dataset can predict RobecoSAM SDG scores of the given companies. As shown in Figure \ref{fig:score distribution} for the RobecoSAM SDG score distribution, we have an imbalanced classification problem because most firms have a neutral score while other classes have few samples. BRF (Balanced Random Forest) is utilized to determine which types of textual data from our dataset best predicts SDG scores. All the text is modelled through BoW (Bag of Words). Robeco provides data for corporate sector classification in 69 industries\footnote{GICS is developed by MSCI and Standard \& Poor's to classify companies to different sectors and industries: \url{https://en.wikipedia.org/wiki/Global_Industry_Classification_Standard}} which can be used as benchmark feature for the classification. GCN (Graph Convolution Networks) is utilized to determine if the corporate graph we created from Wikidata subgraph may help forecast SDG scores beyond textual aspects.

% Another 
% \paragraph{Balanced random forest} 
% \paragraph{Graph Convolutional Network}
% the use of knowledge graphs drastically reduces the need for labeled data, demonstrating the effectiveness of our dataset in the task.
\subsubsection{Generating and forecasting SDG scores}
\textbf{TODO: Maybe remove this section?}
There are 2 main objectives for generating SDG scores: (1) The primary reason for being able to predict MSCI and RSAM scores was to be able to estimate a score for which these providers do not publish one. This can be done via the BRF or GCN. (2) The objective of creating new SDG ratings and providing explanations for those scores is to enhance the present MSCI SDG framework. Through investing in the RobecoSAM SDG framework via classification, we will understand the most important elements they consider for scoring companies. 

However, how to create a more a more transparent, configurable, and scalable SDG framework for a large number of companies remains challenging. SDG scoring index like RobecoSAM primarily focus on the products from which the company generates the majority of its revenue and the general impactful news that has occurred to the company, the evaluation is rather two-dimensional and does not effectively use all of the information that could be deemed relevant or even important for constructing the SDG framework. Therefore, we see an opportunity to enhance their framework by including more dimensions, such as using the additional data we have gathered like Wikidata knowledge graphs, which might represent the relationships (e.g., certain supply chain activities) between the organizations. In this context, generating SDG scores refers to modifying existing SDG ratings to include relevant additional data for scoring the companies more comprehensively by aggregating more information.


% \paragraph{Graph }
% \paragraph{Explaining SDG scores with GNNExplainer}


\begin{table*}[t]
  \centering
  \caption{Sample of summarized key actions for SDG 13: Climate Actions}
  \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{|l|l|p{150mm}|}
    \toprule
    \textbf{company} & \textbf{resource} & \textbf{summarized key actions} \\
    \midrule
    \midrule
    Cleanaway Waste Management Ltd & web   &  by reducing our greenhouse gas emissions , by the responsible management of our landfill gas , and by assisting our customers and the community in managing their waste impacts \\
    \midrule
    Singapore Telecommunications Ltd & report &  undertook a science based targets programme and engaged experts on developing science based targets \\ \midrule
    GlaxoSmithKline PLC & web   &  our climate strategy covers the full value chain of emissions reductions \\ \midrule
    Mapfre SA & web   &  protects the environment through public commitments \\ \midrule
    Carrefour SA & report &  structured its climate action plan around three priority areas \\ \midrule
    Swiss Re AG & report &  we use our existing processes and instruments to address climate - relat \\ \midrule
    Solvay SA & web   &  raising the bar \\ \midrule
    Crown Holdings Inc & web   &  drive climate action throughout our value chain \\ \midrule
    Enagas SA & report &  through efficient use of energy \\ \midrule
    Cie Generale des Etablissements Michelin SCA & report &  taking action both downstream from its operations to ght climate change , conserve natural protect objectives for 2050 to make all the production plants , supply chain operations and raw material and component inputs carbon neutral \\ \midrule
    NextEra Energy Inc & report &  prepare our business to adapt to the effects of climate change \\ \midrule
    Reckitt Benckiser Group PLC & report &  our business strategy sees the macro-trend of climate change as a key factor influencing both our development and society \\ \midrule
    McDonald's Corp & report &  conducting and analyzing scenario modeling to understand the transition and physical risks \\ \midrule
    Prologis Inc & report &  measuring our impact , reducing emissions wherever possible and investing in new technologies and offsets for emissions that , today , cannot be avoided \\ \midrule
    CF Industries Holdings Inc & report &  leverage our unique capabilities to accelerate the worlds transition to clean energy \\ \midrule
    NEL ASA & report &  incorporate sustainability into our strategic decision-making processes \\ \midrule
    SSE PLC & report &  actively and positively advocates to drive accelerated climate action to achieve net zero \\ \midrule
    Catalent Inc & web   &  reducing our carbon footprint \\ \midrule
    Elia Group SA/NV & report &  building our grid \\ \midrule
    Jubilant Pharmova Ltd & web   &  we reduced specific ghg emissions from our facilities year on year , by continuously working on reduction in energy consumption , waste generation , increase in renewable energy share and enhancing the carbon sinks by planting more trees \\
    \bottomrule
    \end{tabular}%
    \end{adjustbox}
  \label{tab:Sample of summarized key actions for SDG 13: Climate Actions}%
\end{table*}%
